Automatic Annotation Augmentation Boosts Translation between Molecules and Natural Language

Recent advancements in AI for biological research focus on integrating molecular data with natural language to accelerate drug discovery. However, the scarcity of high-quality annotations limits progress in this area. This paper introduces LA$^3$, a Language-based Automatic Annotation Augmentation framework that leverages large language models to augment existing datasets, thereby improving AI training. We demonstrate the effectiveness of LA$^3$ by creating an enhanced dataset, LaChEBI-20, where we systematically rewrite the annotations of molecules from an established dataset. These rewritten annotations preserve essential molecular information while providing more varied sentence structures and vocabulary. Using LaChEBI-20, we train LaMolT5 based on a benchmark architecture to learn the mapping between molecular representations and augmented annotations. Experimental results on text-based *de novo* molecule generation and molecule captioning demonstrate that LaMolT5 outperforms state-of-the-art models. Notably, incorporating LA$^3$ leads to improvements of up to 301% over the benchmark architecture. Furthermore, we validate the effectiveness of LA$^3$ notable applications in *image*, *text* and *graph* tasks, affirming its versatility and utility.

==> figures/fig-rewrite-pipeline.tex <==
\begin{figure*}[!ht]
\centering
\includegraphics[width=.8\textwidth]{figures/rewrite_pipeline.pdf}
\caption{
The pipeline for caption augmentation.
Given molecules and their \textcolor{violet}{original captions}, we prompt LLMs to generate \textcolor{oceanboatblue}{augmented captions} by rewriting the original captions. 
The molecule’s SMILES strings are also integrated into this caption generation process to ensure accuracy and relevance.
}
\label{fig:rewrite_pipeline}
\end{figure*}


==> figures/fig-training-pipeline.tex <==
\begin{figure*}[!ht]
\centering
\includegraphics[width=.8\textwidth]{figures/training_pipeline.pdf}
\caption{
\newmodel training pipeline.
}
\label{fig:training_pipeline}
\end{figure*}

